Spectral Survival Analysis

Survival analysis is widely deployed in a diverse set of fields, including healthcare, business, ecology, etc. The Cox Proportional Hazard (CoxPH) model is a semi-parametric model often encountered in the literature. Despite its popularity, wide deployment, and numerous variants, scaling CoxPH to large datasets and deep architectures poses a challenge, especially in the high-dimensional regime. We identify a fundamental connection between rank regression and the CoxPH model: this allows us to adapt and extend the so-called spectral method for rank regression to survival analysis. Our approach is versatile, naturally generalizing to several CoxPH variants, including deep models. We empirically verify our method's scalability on multiple real-world high-dimensional datasets; our method outperforms legacy methods w.r.t. predictive performance and efficiency.

==> Abstract.tex <==
\begin{abstract}
  Survival analysis is widely deployed in a diverse set of fields, including healthcare, business, ecology, etc. The Cox Proportional Hazard (CoxPH) model is a semi-parametric model often encountered in the literature. Despite its popularity, wide deployment, and numerous variants, scaling CoxPH to large datasets and deep architectures poses a challenge, especially in the high-dimensional regime.  We identify a fundamental connection between rank regression and the CoxPH model: this allows us to adapt and extend the spectral method for rank regression to survival analysis. Our approach is versatile, naturally generalizing to several CoxPH variants, including deep models. We empirically verify the ability of our method to scale on multiple real-world high-dimensional datasets, including a three-dimensional CT scan dataset that could not be handled by SOTA survival analysis methods without the use of dimensionality reduction techniques. Moreover, we show by executing a full-batch gradient descent our method outperforms legacy methods which require additional multi-modal input and expert annotation.
\end{abstract}

==> Conclusion.tex <==
\section{Conclusion}
We have shown how a spectral method motivated by ranking regression can be applied to scaling survival analysis via CoxPH and multiple variants. Extending this model to other variants of CoxPH and DeepSurv is an interesting open direction. The \textsc{Spectral} outperforms SOTA methods on various high-dimensional medical datasets such as genetic and cancer datasets, and, therefore, could benefit the medical care field. Although \textsc{Spectral} shows significant improvement in complex datasets, it does not improve the performance of SOTA methods in the low-dimensional regime. We leave the exploration for future work. The code will be released after publication.

==> Experiments.tex <==

\section{Experiments}
\label{sec: experiments}
\begin{table*}[!t]
\begin{center}
% \begin{small}
% \begin{sc}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{Metrics} & \multirow{2}{*}{Algorithms} & \multicolumn{3}{c}{\bf Low-dimension datasets}& \multicolumn{3}{c}{\bf High-dimension datasets}\\
& & SUPP &  META &  WHAS &  DBCD &  DLBCL &  VDV\\
\hline
\multirow{7}{*}{\bf CI $\uparrow$}&DeepHit & 0.566±0.032 & 0.585±0.023 & 0.823±0.013 & 0.691±0.023& 0.617±0.061 & 0.647±0.105\\
&DeepSurv & \textbf{0.586±0.006} & 0.635±0.006 & 0.830±0.017 & 0.642±0.042 & 0.595±0.032 & 0.505±0.033\\
&FastCPH & 0.555±0.003 &  0.657±0.006 & 0.815±0.010 & 0.724±0.109 & 0.574±0.069 & 0.567±0.065\\
&CoxTime & 0.564±0.003 & 0.655±0.008 & 0.787±0.013 &  0.658±0.025 & 0.556±0.058 & 0.593±0.020\\
&CoxCC & 0.577±0.004 & \textbf{0.678±0.007} & 0.815±0.006 & 0.628±0.029 & 0.596±0.074 & 0.596±0.125 \\
&NMTLR & 0.506±0.021 & 0.595±0.006 & 0.793±0.020 & 0.716±0.023 & 0.577±0.045& 0.536±0.139 \\
&Spectral  & 0.557±0.019 & 0.600±0.016  & \textbf{ 0.835±0.023} & \textbf{0.724±0.007} & \textbf{0.625±0.065} & \textbf{0.716±0.050} \\
\hline
% \multirow{7}{*}{\bf IBS$ \downarrow$}&DeepHit &0.263±0.011 &0.173±0.007 &0.140±0.005 & 0.307±0.029 & 0.236±0.004&0.244±0.016\\
% % DeepHit \ding{70} &0.250 &0.184 &0.162 & 0.263 & 0.251&0.250 \\
% &DeepSurv     &0.212±0.001 &0.184±0.003& \textbf{0.108±0.010}& 0.176±0.024 & 0.255±0.029&0.243±0.015\\
% % DeepSurv\ding{70}      &0.191 &0.167 &0.192 & 0.167 & 0.245&0.41\\
% &FastCPH   &0.214±0.002 &0.188±0.004 &0.131±0.009 & 0.175±0.076 & 0.403±0.043&0.234±0.026 \\
% &CoxTime  &0.210±0.001 &0.161±0.004 &0.145±0.012 & \textbf{0.148±0.011} & 0.346±0.050&0.283±0.019\\
% &CoxCC  &\textbf{0.209±0.002} &\textbf{0.158±0.003} &0.137±0.004 & 0.236±0.018 & \textbf{0.178±0.021}&0.294±0.037\\
% &NMTLR  &0.234±0.004 &0.176±0.005 &0.118±0.005 & 0.251±0.031 & 0.226±0.030& 0.263±0.060 \\
% &Spectral & 0.217±0.003&0.200±0.010 &0.131±0.016 & 0.308±0.014 & 0.334±0.046 &\textbf{0.209±0.021}  \\
% \hline 
\multirow{7}{*}{\bf iAUC $\uparrow$}&DeepHit  & 0.499±0.033& 0.667±0.018&0.793±0.046 & 0.728±0.031 & 0.617±0.061& 0.647±0.105\\
% DeepHit \ding{70} & & & & & & \\
&DeepSurv & 0.586±0.006&0.688±0.009 & 0.896±0.031& 0.661±0.044 & 0.667±0.037& 0.505±0.033\\
% DeepSurv\ding{70} & & &0.543 & & & 0.5\\
&FastCPH &0.579±0.005 &0.691±0.006 &0.876±0.012 & 0.677±0.131&0.609±0.097& 0.576±0.070\\
&CoxTime  & 0.596±0.004& \textbf{0.728±0.013}& 0.855±0.014& 0.706±0.028& 0.556±0.058& 0.569±0.059\\
&CoxCC  &\textbf{0.610±0.005} & 0.723±0.011&0.849±0.010 & 0.628±0.029&  0.629±0.087& 0.612±0.152\\
&NMTLR  &0.538±0.023 &0.703±0.009 &\textbf{0.911±0.006} & 0.608±0.033& 0.585±0.041 & 0.423±0.214\\
&Spectral  &0.584±0.027 &0.647±0.020 &0.890±0.015 & \textbf{0.734±0.016}& \textbf{0.698±0.076}& \textbf{0.762±0.046} \\
\hline
\end{tabular}}
% \end{sc}
\caption{Comparison of \textsc{Spectral} with other state-of-the-art (SOTA) hazard models on 1D datasets w.r.t CI and iAUC, with standard deviation computed over $k$-folds (see Table~\ref{table: Datasets}). RMSE is reported in the supplement. Results indicate suboptimal performance of \textsc{Spectral} on low-dimension datasets (Support, Metabric, and WHAS). We attribute this to the simplicity of low-dimension datasets, where simple MLPs guided by partial likelihood loss suffice. However, for high dimensional datasets (DBCD, DLBCL, and VDV), \textsc{Spectral} outperforms baselines. We attribute this to the increased complexity of high-dimension manifolds and sparse data distribution, which requires intrinsic hazard scores for appropriate mappings. \textsc{Spectral} demonstrates significant improvements in CI and iAUC.} 
\label{table: performance for vectors}
% \end{small}
\end{center}
\end{table*}
\subsection{Experiment Setup}
\noindent{\bf Datasets.} We conduct experiments on seven publicly available real-world datasets summarized in Table.~\ref{table: Datasets} which follow Fig.~\ref{fig: illustration}: six vector features and one is a three-dimension CT scan dataset (Lung1). We also generated a synthetic counting process arrival rate dataset, following the scenario of \cite{chen2023gateway}. Additional details about each dataset are provided in App.~\ref{app: experiment details}. We use 10\% of each dataset as a hold-out test set and conduct $k$-fold cross-validation on the training set to determine hyperparameters, with $k$ indicated in Table~\ref{table: Datasets}. 


%We train multi-layer perception on one-dimensional datasets and a 3D CNN on Lung1. 
{\bf \noindent Survival Analysis Regression Methods.} We implement our spectral method (\textsc{Spectral}) and compare it against six SOTA survival analysis regression competitors. Four are continuous-time methods (\textsc{DeepSurv} \cite{Katzman2018DeepSurvPT}, \textsc{CoxTime} \cite{CoxTimeCC}, \textsc{CoxCC} \cite{CoxTimeCC}, \textsc{FastCPH} \cite{yang2022fastcph}), and regress the hazard rate from features.  Two are discrete-time methods (\textsc{DeepHit} \cite{lee2018deephit} and \textsc{NMTLR} \cite{NMTLR}); they split time into intervals and treat the occurrence of an event in an interval as a classification problem, thereby estimating the PMF. For all methods, except \textsc{FastCPH}, we use the DNN architectures shown in the last column Table.~\ref{table: Datasets}: this is a 6-layer 3D CNN for Lung1 data, and MLP with 2-6 layers, for the remaining datasets (see also App.~\ref{app: experiment details}); we treat the number of layers as a hyperparameter to be tuned. 
FastCPH has a fixed network structure, LassoNet~\cite{lassonet21}: we set the number of layers to 2-6 and again treat depth as a hyperparameter. As LassoNet is incompatible with the 3D dataset Lung1, we do not report experiments with FastCPH on this dataset. For all the methods, we explore the same hyperparameter spaces. Additional implementation details are provided in App.~\ref{app: experiment details}.


\noindent\textbf{Legacy Methods.}  Aside from the implemented methods, we also report the performance of four legacy methods executed on  Lung1; we do not re-execute these methods. We note that (a) three of these methods use additional features beyond CT scans and (b) none can operate on the entire scan, but rely on dimensionality reduction methods to process the input. Details are provided in App.~\ref{app: experiment details}.



{\bf \noindent Hyperparameter Search.} Optimal hyperparameters are selected based on $k$-fold cross-validation on the dataset, using early stopping; we use CI as a performance metric (see below). The full set of hyperparameters explored is described in App.~\ref{app: experiment details}. % As we apply early-stopping, we evaluate the method with the checkpoint that shows the best validation performance (CI).




{\bf \noindent Metrics:}
We adopted the 3 commonly used metrics: C-Index (CI, higher is better $\uparrow$), integrated AUC (iAUC,  higher is better $\uparrow$), and RMSE (lower is better $\downarrow$). All three are defined formally in App.~\ref{app: experiment details}.






\subsection{Results}
\noindent{\bf 3D Lung1 dataset.}
In Table.~\ref{table: Lung1 performance.}, we first list the performance of legacy methods on the benchmark Lung1 dataset, as reported in the respective papers. This is followed by the five competitors we implement for Lung1, along with \textsc{Spectral}. We measure predictive performance in terms of CI, RMSE, and iAUC. \textsc{Spectral} outperforms both legacy methods as well as all competitors w.r.t.~all metrics. We note that legacy methods have access to additional features beyond CT scans. Moreover, these methods rely on dimensionality reduction techniques such as subsampling patches (some under the supervision of human experts) to process the CT scan input. Similarly, none of the competitor methods can process the entire CT scan and require using mini-batch SGD, which drops samples from the objective, e.g., the risk set of CoxPH in \eqref{eq: CoxPH plik} would become a true subset of the original $\mathcal{R}(T_i)$. 
% Though we report time and memory on the A100,  \textsc{Spectral} can even be executed on an NVIDIA V100 (with 32Gb of RAM); all other methods fail even with 10\% mini-batches. 
The time spent by \textsc{Spectral} is around ten times compared to the competitor methods. However, operating on 10\% mini-batches reduces the time complexity to 10\% with the batch-based partial likelihood. Thus,  the time required by other methods to operate on a full batch would be of the same magnitude per epoch.
We evaluate the DeepSurv and \textsc{Spectral} with different batch sizes as in Fig.~\ref{fig: lung1}. We observe the \textsc{Spectral} outperforms DeepSurv with all batch sizes, and it scales in terms of memory.  DeepSurv runs out of memory when the mini-batch exceeds 10\%  over an NVIDIA A100 with 80Gb of RAM. Both methods show better performance with larger batch sizes.
%
%In contrast, \textsc{Spectral} is able to run \emph{on the full dataset} on the V100. Moreover, it outperforms both legacy methods as well as all competitors w.r.t. CI and iAUC.
%For the Lung1 dataset, we use a 6-layer 3D-CNN to compare against different methods. We first introduced the SOTA work specifically focusing on Lung1. Due to the large volume of 3D data, all of them either work on extracted 2D radiomic images, patches, or slices of Lung1 CT images. As they are not generally focusing on the hazard model as our paper is, we only report the results from their papers regarding the Lung1 dataset \cite{zhu2016deepconvsurv, Haar2019, Brag2023, ZHENG2023109483}.

%\noindent{\bf Reported Lung1-specific SOTA methods.} As we can see from the table~\ref{table: Lung1 performance.}, compared with the reported results (\cite{zhu2016deepconvsurv, Haar2019, Brag2023, ZHENG2023109483}), our method on whole image outperforms their methods even though they have multi-modal inputs \cite{zheng2023cancergroups, Brag2023, Haar2019}. Moreover, \textsc{Spectral} outperforms \citet{zhu2016deepconvsurv} which applies \textsc{DeepSurv} to patches with pathologists' manual annotation. Thus, it is necessary to work on the whole images rather than partial images such as patches, slides, or cubes, to fully utilize the information from the dataset. Moreover, it is possible to combine multi-modal inputs with the proposed \textsc{Spectral} to further improve the performance. But we leave the empirical exploration for future work.

%\noindent{\bf General SOTA hazard models.} Then, we compare \textsc{Spectral} against the other five SOTA hazard models. The ideal case is to run full-batch GD with each method so that the original partial likelihood loss such as Eq.~\eqref{eq: DeepSurv Loss} could be computed to conduct GD. However, as we mentioned, the siamese network essence in survival analysis limits the scalability as we need to compute identical network parameters on all the samples simultaneously. Thus, all of the baseline methods run out of memory under the full batch regime on NVIDIA V100-SXM2-32GB. Moreover, none of the baseline methods can run with $10\%$ mini-batch. Thus, we implemented the experiments again on the NVIDIA A100 80G, where we failed again with a mini-batch containing $50\%$ of the dataset. Thus, we report the $10\%$ cases, where \textsc{CoxTime} and \textsc{CoxCC} still failed due the memory insufficiency as they require a sufficiently large at-risk sample set to approximate the numerator term of the partial likelihood. 

%The results show the small mini-batches update hinders the performance of the baselines as they are optimizing the networks towards only a fraction of the original partial likelihood. Meanwhile, our Theorem allows us to directly approach the closed-form solution (intrinsic scores) of the original partial likelihood, and the subsequent regression-type model can learn the mapping from feature space to optimum intrinsic scores with any batch size. Although \textsc{Spectral} shows significant improvement in CI and iAUC, the IBS is sub-optimal, and we attribute it to the way we calculate the survival function with the Breslow estimator, and we observe the survival function does not start from 1 at $t=0$ due to missing data close to the initial point. Thus, further improving the estimator for survival function may improve the IBS.





% \begin{table}
%   \caption{Frequency of Special Characters}
%   \label{tab:freq}
%   \begin{tabular}{ccl}
%     \toprule
%     Non-English or Math&Frequency&Comments\\
%     \midrule
%     \O & 1 in 1,000& For Swedish names\\
%     $\vpi$ & 1 in 5& Common in math\\
%     \$ & 4 in 5 & Used in business\\
%     $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
%   \bottomrule
% \end{tabular}
% \end{table}


% \begin{table*}
%   \caption{Some Typical Commands}
%   \label{tab:commands}
%   \begin{tabular}{ccl}
%     \toprule
%     Command &A Number & Comments\\
%     \midrule
%     \texttt{{\char'134}author} & 100& Author \\
%     \texttt{{\char'134}table}& 300 & For tables\\
%     \texttt{{\char'134}table*}& 400& For wider tables\\
%     \bottomrule
%   \end{tabular}
% \end{table*}


\noindent\textbf{Synthetic Ads Dataset.} The Synth Ads dataset differs as it models a counting process, in which an ad click event is regressed from the history of past impressions made to a user (see App.~\ref{app: extensions}). In Fig.~\ref{fig: ads}, we plot the time and performance of DeepSurv and \textsc{Spectral} against different amounts of samples. We observe that \textsc{Spectral} always outperforms the DeepSurv counterparts in AUC, and the time cost of \textsc{Spectral} is less dependent on the sample size. Specifically, when there are $100$ journeys DeepSurv spends 60\% less time than \textsc{Spectral}. However, when there are $10,000$ journeys DeepSurv spends $100 \times$ time than \textsc{Spectral}.

\noindent\textbf{1D Datasets.}
Our remaining datasets pose less of a challenge in terms of memory requirements. Thus, all competitors run under the full-batch regime. We can thus analyze the performance of \textsc{Spectral} against other SOTA hazard models under the same regime. 
Table.~\ref{table: performance for vectors} shows the two metrics on all algorithms and datasets, while the RMSE is in App.~\ref{app: experiment details}. \textsc{Spectral} shows suboptimal performance on low-dimensional datasets (Support, Metabric, and WHAS), that have between 5--34 features (see also Table.~\ref{table: Datasets}). However, it consistently outperforms the baselines on CI and iAUC on higher-dimension datasets (DBCD, DLBCL, and VDV), whose dimension $d$ ranges between 4705--7399. 
%


\noindent\textbf{Limitations.} 
In short, with sufficient samples, the low-dimension datasets can be handled by simple MLPs directly guided by the partial likelihood loss, as the objective has a simple manifold. In contrast, high-dimension datasets live on more complex manifolds with sparse data points, where intrinsic hazard scores are needed for appropriate mappings, and thereby avoid overfitting. As the memory complexity becomes $\min{(O(n^2), O(PB))}$ instead of $O(PnB)$ with the spectral method, the model will be less effective in the case where a simple shallow network suffices ($P<\frac{n}{B}$, i.e. $PnB < n^2$), such as datasets with fewer features like SUPPORT, WHAS. 




==> Intro.tex <==
\section{Introduction}
\label{sec: intro}
The goal of survival analysis is to regress the distribution of event times, given a set of samples, along with observations of associated event times. Survival analysis is widely deployed in a diverse set of fields, including healthcare \cite{murtaugh1994primary, Ganssauge2017, Zupan1999}, business \cite{FADER200776}, economics \cite{danacica2010using}, and ecology \cite{lebreton1993statistical}, to name a few. A prototypical example in healthcare involves regressing the time until a significant event in a patient's history occurs (e.g., the onset of a disease, the emergence of a symptom, etc.) based on the patient's medical records \cite{Ganssauge2017, Zupan1999}. Another application includes the regression of counting process arrival rates from, e.g., past events or other temporal features  \cite{AalenBook,chen2023gateway}.  
%
Methods implementing regression in this setting are numerous and classic~\cite{CoxPH1972, EH2021, Wei1992TheAF}. Among existing methods, the Cox Proportional Hazard (CoxPH) model is a popular semi-parametric model. The ubiquity of CoxPH is evidenced not only by its wide deployment and use in applications \cite{lane1986application, liang1990applicationepid, wong2011applicationchurn}, but also by its numerous extensions \cite{subgroupreweight, hu2021subgroup},  including recently proposed deep learning variants \cite{Katzman2018DeepSurvPT, CoxTimeCC}.

Despite its widespread use, CoxPH and its variants lack scalability, especially in the high-dimensional regime. The scalability issue comes from the partial likelihood that CoxPH optimizes, which \emph{incorporates all samples in a single term in the objective}. Previous works reduce the computational complexity of CoxPH variants through mini-batching\cite{CoxTimeCC, zhu2016deepconvsurv}, but it leads to biased gradient estimation and reduces performance in practice. Matters are only worse in the presence of deep models, which require loading both the samples and $O(n)$ identical copies of the neural network in the penalty to compute the loss, where $n$ is the size of the dataset. This significantly increases the costs of training in terms of both computation and memory usage; conversely, there is a limitation on the model architecture size as well as the size and dimensions of the training dataset that can be combined with CoxPH and its deep variants. \emph{As a result, all present deployments of methods with original data input are limited to shallow networks} \cite{Katzman2018DeepSurvPT, coxnnet2018cox, CoxTimeCC, YAO2020101789, SurvCNN21, yin2022convolutional, zhu2016deepconvsurv} or \emph{require the use of subsampling and dimensionality reduction techniques}~\cite{SurvCNN21,wang2018comprehensive} to be deployed in realistic settings.  


% due to the concavity of the log function in the denominator, i.e., $
% \mathbb{E}\left[\log\left(\sum X_i\right)\right] \leq \log\left(\mathbb{E}\left[\sum X_i\right]\right)$.


%For example, \citet{Katzman2018DeepSurvPT} propose DeepSurv, replacing linear models with neural networks, yet their application is limited to shallow MLPs and small datasets for the survival analysis tasks.


\fussy
%As CoxPH optimizes the partial likelihood across all samples, itself and all its variants do not readily scale, neither to  large inputs nor to large models. For instance, the optimization of the deep version of CoxPH, i.e., DeepSurv \cite{Katzman2018DeepSurvPT}, inevitably induces the siamese neural networks (SNN) \cite{chicco2021siamese} over all samples. %\footnote{SNN consists of a pair of or multiple neural networks that share structure and weights, which serve similar functionality} Although CoxCC claims their method enables mini-batch stochastic gradient descent, the sufficiently large sampled risked set still hinders the scalability. This results in expensive computation and memory costs during training in the forward and backward propagation. In practice, this limits the application of CoxPH to small networks and datasets \cite{Katzman2018DeepSurvPT, tang2022soden}.

In this work, we leverage an inherent connection between CoxPH and \emph{rank regression} \cite{yildiz20a,yildiz21a,Burges2005LearningTR,Cao2007LearningTR,yildizTKDD}, i.e., regression of the relative order of samples from their features, using ranking datasets. Recently, a series of papers \cite{maystre2015fast,yildiz20a,yildiz21a,yildizTKDD} have proposed spectral methods to speed up ranking regression and to deal with memory requirements similar to the ones encountered in survival analysis. Our main contribution is to observe this connection and adapt these methods to the survival analysis domain. % by solving the placket-Luce model efficiently without inducing SNN. Thus, in response to the scalability challenge, we propose a Deep Spectral Learning (DSL) method. This empowers deep Cox models stochastic gradient descent, where a single sample is processed each time, This method improves both scalability and accuracy. Our method applies to multiple hazard models. For instance, the method can be applied to a more general setting where multiple class-specific baseline functions are learned for better modeling instead of assuming a common baseline function. Besides, the setup can be directly applied to grant previous hazard models scalability. 
Overall, this paper has four contributions: 
\begin{itemize}
    \item We identify a fundamental connection between rank regression and survival analysis via the CoxPH model and its variants. 
    \item We adapt and extend the spectral method by Yildiz et al. \cite{yildiz21a} to CoxPH. To the best of our knowledge, ours is the first spectral approach used to attack survival analysis regression. %Therefore, the optimization problem shifts from optimizing the partial likelihood to regressing the intrinsic scores, enabling the usage of SGD and scalability to large datasets. 
    \item We show that this approach is versatile: in particular, it naturally generalizes to several variants of CoxPH, including deep models, that are extensively used in applications of survival analysis. 
    \item We empirically verify the ability of our method to scale on multiple real-world high-dimensional datasets, including a three-dimensional CT scan dataset. We can scale deep CoxPH models (DeepSurv) and outperform state-of-the-art methods that rely on dimensionality reduction techniques, improving both memory and running time performance (see Fig.~\ref{fig:teaser}).
\end{itemize}
From a technical standpoint, we extend the analysis of Yildiz et al. \cite{yildiz21a} by incorporating weights in the loss, and showing that its stationary points can still be expressed as solutions of a continuous Markov Chain. This extension is crucial in tackling a broad array of CoxPH variants: we show how to address the latter via a novel alternating optimization technique, combining spectral regression with a Breslow estimate of baseline hazard rates.

==> Method.tex <==

\section{A Spectral Method}
\label{sec: method}
%\subsection{Decoupling Samples via Spectral Methods}
As discussed in Sec.~\ref{sec: preliminaries}, CoxPH optimizes the partial likelihood (Eq.~\eqref{eq: CoxPH plik}). However, this likelihood \emph{incorporates all samples in a single batch/term in the objective}. This is exemplified by Eqs.~\eqref{eq:nll} and~\eqref{eq: DeepSurv Loss}: all samples $j\in\mathcal{R} (T_i)$ need to be included in the loss when computing the term corresponding to sample $i$.  This is exacerbated in the case of DeepSurv (Eq.~\eqref{eq: DeepSurv Loss}), as it requires loading both the samples but also $|\mathcal{R}(T_i)|$ identical copies of the neural network in the penalty to compute the loss.\footnote{This structure is also referred to as a Siamese network loss~\citep{chicco2021siamese} in the literature} This makes backpropagation extremely expensive in terms of both computation and memory usage. In turn, this significantly limits the model architectures as well as the number and dimensions of the datasets that can be combined with DeepSurv and the other extensions mentioned above. As a result, all present deployments of these methods with original data input are limited to shallow networks \cite{Katzman2018DeepSurvPT, coxnnet2018cox, CoxTimeCC, YAO2020101789, SurvCNN21, yin2022convolutional, zhu2016deepconvsurv} or require the use of subsampling and dimensionality reduction techniques~\cite{SurvCNN21,wang2018comprehensive} which inevitably lead to information loss.  %For example, \cite{Katzman2018DeepSurvPT} propose DeepSurv, replacing linear models with neural networks, yet their application is limited to shallow MLPs and small datasets for the survival analysis tasks.

We directly address this issue in our work. In particular, we show that spectral methods~\cite{maystre2015fast, yildiz20a,yildiz21a} can be used to decouple the minimization CoxPH and DeepSurv losses from fitting the neural network. Thus, we convert the survival analysis problem (likelihood optimization) to a regression problem, fitting the neural network to intrinsic scores that minimize the loss. Crucially, these scores can be efficiently computed via a spectral method, while fitting can be done efficiently via stochastic gradient descent on \emph{a single sample/score} at a time. As we will show in Sec.~\ref{sec: experiments}, this yields both time and memory performance dividends, while also improving the trained model's predictive performance.  By leveraging Theorem~\ref{thm: ss} we can extend the spectral method to scale other models beyond DeepSurv, such as AFT \cite{chen2003accelerated}, and Heterogeneous CoxPH~\cite{hu2021subgroup}, as well as to regress the arrival rate of a counting process. We focus in this section on CoxPH/DeepSurv for brevity, and present such extensions in detail in Appendix~\ref{app: extensions}.


% To make the following method compatible with both DeepSurv and CoxPH, we unify the expression of both the exponential linear model $f(\vx_i)=e^{\mtheta^\top x_i}$ and neural network with parameter as $h_{\mtheta}(\cdot)$. However, different from \cite{yildiz21a}, we proposed the weighted spectral method that enables the extension of our method.

% First, we reformulate the problem in CoxPH/DeepSurv with intrinsic score approximation constraints
% \begin{align}\label{eq: deepsurv problem}
%     \max_{\vpi, \mtheta } \PL(\dataset|\mtheta)= &\prod_{i=1}^n\left[   \frac{ h_{\mtheta} ( \vx_i) }{\sum_{j\in \mathcal{R}_i}  h_{\mtheta}( \vx_j)}\right]^{\Delta_i}\\
%     s.t. \quad \vpi = & h_{\mtheta}(\mX), \vpi\geq 0,\nonumber
% \end{align}

% Comparing \eqref{eq: deep spectral problem} with \eqref{eq: deepsurv problem}, we observe that the partial likelihood is equivalent to PL model in ranking if all the observations are actual events rather than censoring, i.e., $\Delta_i=1, \forall i \in [n]$, and $\mathcal{S}\equiv\mathcal{R}$.

\subsection{Regressing Weighted CoxPH \& DeepSurv}
\label{subsec: weighted deepsurv}
We describe here how to apply the spectral methods introduced by \cite{maystre2015fast} and  \cite{yildiz21a} to the survival analysis setting; we first present this in the context of the weighted CoxPH model and then show how it can be extended to the array of hazard models presented in App.~\ref{app: extensions}. Our main technical departure is in handling heterogeneity in the loss, as induced by weights, which \cite{yildiz21a} do not consider. This is crucial in generalizing our approach to CoxPH extensions, which are also technically involved, and incorporating alternating between regression and  Breslow estimate of the baseline hazard. %(Eq.~\eqref{eq: smoothing Breslow}). %moreover, we further propose the Weighted DeepSurv which generalizes the method to include an . Note that as in the \cite{yildiz21a}, we approximate the intrinsic scores $\vpi$ with a function $h_{\mtheta}$ directly, skipping the exponential term.


%\noindent{\bf Weighted DeepSurv}. 
\noindent{\bf Reduction to a Spectral Method}.
We apply the spectral approach by \cite{yildiz21a} to minimize the following general negative-log likelihood:
\begin{align}\label{eq: reweight deepsurv nll}
   \NLL(\dataset,\mtheta) =  \frac{1}{n}\sum_{i=1}^n {\Delta_i}\left(\log\sum_{j\in \mathcal{R}_i}\mW_{ji} \tilde{h}_{\mtheta}(\vx_j)- \log  \mW_{ii} \tilde{h}_{\mtheta}(\vx_i) \right).
\end{align}
where we define $\mathcal{}{R}_i \equiv \mathcal{R}(T_i)$ for simplicity. Setting $ \tilde{h}_{\mtheta}(\vx)\equiv e^{\mtheta^\top \vx}$, we obtain the  Weighted CoxPH model;  setting it to be $ \tilde{h}_{\mtheta}(\vx)\equiv e^{\tilde{h}_{\mtheta}(\vx)}$, where ${h}_{\mtheta}(\vx)$ a deep neural network we obtain a weighted version of DeepSurv; finally, setting the weights to be one yields the standard CoxPH/DeepSurv models. Parameters in all these combinations can be learned through our approach.
% \begin{align}\label{eq: weight deepsurv problem}
%     \max_{\vpi, \mtheta } \PL(\dataset|\mtheta)= &\prod_{i=1}^n\left[   \frac{ h_{\mtheta} ( \vx_i) }{\sum_{j\in \mathcal{R}_i}  h_{\mtheta}( \vx_j)}\right]^{\Delta_i}\\
%     s.t. \quad \vpi = & h_{\mtheta}(\mX), \vpi\geq 0,\nonumber
% \end{align}

Our goal is to minimize this loss. Following \cite{yildiz21a}, we reformulate this minimization as the following constrained optimization problem  w.r.t. $\vpi$, $\mtheta$:
 \begin{subequations}\label{eq: deepsurv problem}
      \begin{align}
     \text{Minimize}:& \sum_{i=1}^n {\Delta_i} \left(\log\sum_{j\in \mathcal{R}_i}\mW_{ji} \vpi_j- \log  \mW_{ii} \vpi_i \right)\\
     \text{subj.~to}: & \quad \vpi =  \tilde{h}_{\mtheta}(\mX), \vpi\geq 0,
 \end{align}
  \end{subequations}
where $\mX\coloneqq [\vx_1,\dots, \vx_n]^\top\in \R^{n\times d}$, $\tilde{h}_{\mtheta}\in \R^n_+$ is a map from this matrix to the images $ \tilde{h}_{\mtheta}(\vx_i)$ of every sample $\vx_i$,  $\vpi=[\vpi_1, \cdots, \vpi_n]^n \in \R_+^n$, and auxiliary variables $\vpi_i\in\R_+$, $i\in [n]$, are \emph{intrinsic scores} per sample: they are proportional to the probability that a sample $i$ experiences an event before other at-risk samples. 
We solve this equivalent problem via the Alternating Directions Method of Multipliers (ADMM) \cite{boyd2011admm}. In particular, 
we define the augmented Lagrangian of this problem as:
\begin{align}\label{eq:weighted deepsurv lagrangian}
\begin{split}
    \loss(\vpi,\mtheta,\vu)\equiv & \sum_{i=1}^n {\Delta_i}\left(\log\sum_{j\in \mathcal{R}_i}\mW_{ji} \vpi_j- \log \mW_{ii} \vpi_i  \right)\\
    &+\vu^\top (\vpi - \tilde{h}_{\mtheta}(\mx))+\rho \mathcal{D}_{KL}(\vpi||h_{\mtheta}(\mx)),
    \end{split}
\end{align}
where $\mathcal{D}_{KL}(\cdot||\cdot)$ is the KL-divergence. Subsequently, ADMM proceeds iteratively, solving the optimization problem in Eq.~\eqref{eq:weighted deepsurv lagrangian} in an alternating fashion, optimizing along each parameter separately:
\begin{subequations}
\label{eq:admm}
\begin{align}
\vpi^{(k+1)}=&\argmin_{\vpi\geq 0} \loss(\vpi,\mtheta^{(k)},\vu^{(k)}) \label{lin pi}\\
    \mtheta^{(k+1)}=&\argmin_{\mtheta} \loss(\vpi^{(k+1)},\mtheta,\vu^{(k)}) \label{lin theta}\\
    \vu^{(k+1)}=& \vu^{(k)} +\rho (\vpi^{(k+1)} - h_{\mtheta^{(k+1)}}(\mx)). \label{dual params}
\end{align}  
\end{subequations}
% where the closed-form solution \eqref{lin pi} can be obtained according to Theorem~\ref{thm: ss} followed by the spectral method.
This approach comes with several significant advantages. First, Eq.~\eqref{lin pi}, which involves the computation of the intrinsic scores, can be performed efficiently via a spectral method. Second, Eq.~\eqref{lin theta} reduces to standard regression of the model w.r.t the intrinsic scores, which can easily be done via SGD, thereby decoupling the determination of the intrinsic scores (that involves the negative log-likelihood) from training the neural network. Finally, Eq.~\eqref{dual params} is a simple matrix addition, which is also highly efficient. We describe each of these steps below. 


\noindent\textbf{Updating the Intrinsic Scores (Eq.~\eqref{lin pi}).} We show here how the intrinsic score computation can be accomplished via a spectral method. To show this, we first prove that the solution to ~\eqref{lin pi} can be expressed as the steady state distribution of a certain Markov Chain (MC): 
\begin{theorem}\label{thm: ss}
The stationary point of equation~\eqref{lin pi} satisfies the balance equations of a continuous-time Markov Chain 
 with transition rates 
\begin{equation}\label{eq: P}
\mP_{ji}(\vpi)=
\begin{cases}
\mu_{ji}+\frac{2\vpi_i \sigma_i(\vpi) \sigma_j(\vpi)}{\sum_{t\in [n]_-}\vpi_t \sigma_t(\vpi)-\sum_{t\in [n]_+}\vpi_t \sigma_t(\vpi)} & \textit{if } j \in [n]_+\land i\in [n]_- \\
\mu_{ji} & \textit{otherwise},\\
\end{cases}
\end{equation}
where  $[n]_{+}=\{i:\sigma_i(\vpi)\geq 0\}$, $[n]_{-}=\{i:\sigma_i(\vpi)\leq 0\}$, and
\begin{align}
\sigma_i(\vpi)= &\rho \frac{\partial D_p(\vpi||\tilde{h}_{\mtheta}(\mx))}{\partial \vpi_i}+u^{(k)}_i, \quad \mu_{ji}=\sum_{\ell\in W_i\cap L_j}\Delta_\ell \left(\frac{\vW_{j,\ell}}{\sum_{t\in R_\ell} \vW_{t,i} \vpi_t}\right), \label{eq: sigma and mu}\\
W_i=\{\ell|i\in & R_\ell,  i=\argmin_{j\in R_\ell} O_j\},\quad L_i=\{\ell|i\in R_{\ell},i \neq \argmin_{j\in R_\ell} O_j\}.
% \sum_{\ell\in W_i\cap L_j}\Delta_\ell \left(\frac{\mW_{j\ell}}{\sum_{t\in R_\ell} \mW_{t\ell} \vpi_t}\right)=
% 
\end{align}
\end{theorem}
We prove this in Appendix~\ref{app:proof}.  
This is the equivalent of Theorem~4.1 in \cite{yildiz21a}, applied to our setting. A key technical difference is the presence of weights, which changes the transition rates and structure of the MC as well as how the balance equations are satisfied.
%

As indicated in \cite{yildiz21a,maystre2015fast}, Theorem~\ref{thm: ss} can be used to obtain a solution to \eqref{lin pi}. This is done by applying the following iterations:
\begin{align}
    \vpi^{(k+1)}=\mathrm{ssd}(\mP(\vpi^{(k)})),\label{eq:ssd}
\end{align}
where $\mP(\vpi^{(k)})$ is the transition matrix given by Theorem~\ref{thm: ss}, and $\mathrm{ssd}(\cdot)$ is an operator that returns the steady state distribution of the corresponding continuous-time MC.  This can be computed, e.g., using the power method \cite{Kuczynski1992power}.


%Thus, by spectral methods, we obtain the steady state distribution of the MC, i.e., the optimal intrinsic scores $\vpi$ that minimize the partial likelihood. More importantly, by regressing the intrinsic scores, the problem turns from \emph{traditional survival analysis} to \emph{regression}, which is scalable and will be compatible with modern regression-oriented techniques.

\noindent\textbf{Fitting the Model (Eq.~\eqref{lin theta}).}  In Appendix~\ref{app:max entropy}, we show that Eq.~\eqref{lin theta} is equivalent to the following problem:
%\begin{align}
 $   \min_{\mtheta} \sum_{i=1}^n\left( - \vu_i^\top h_{\mtheta}(\vx_i)+\rho \vpi_i^{(k+1)}\log (\tilde{h}_{\mtheta}(\vx_i))\right).$
%\end{align}
%This equivalence is shown
%
This is a standard max-entropy loss minimization problem, along with a linear term, and can be optimized via standard stochastic gradient descent (SGD) over the samples.

\noindent\textbf{Updating the Dual Variables (Eq.~\eqref{dual params}).}
The dual parameters are updated by adding the difference between intrinsic scores and the prediction of the updated network.

\begin{algorithm}[t]
\caption{Spectral Weighted Survival Analysis}
\label{algo: ADMM}
\begin{algorithmic}[1]
\Procedure{\textsc{SpectralWeightedSA}}{$\vpi, \mtheta, \vu, \mW, \dataset$}
    \State Initialize $\hat{\vpi}\gets \frac{1}{n} \vone$; $ \vu \gets \vzero$
    \Repeat
    \State $\vpi\gets \textsc{IterativeSpectralRanking}(\rho,\vpi,\vu, \hat{\vpi}, \mW)$ %\textit{via Theorem~\ref{thm: ss}}$
    \State $\mtheta \gets \textit{SGD over } \eqref{lin theta}$
    \State $\hat{\vpi} \gets \tilde{h}_{\mtheta}(\mx)$
    \State $\vu \gets \vu + \rho(\vpi-\hat{\vpi})$
    \Until{Convergence}
\State \Return $\vpi, \mtheta$
\EndProcedure
\Procedure{IterativeSpectralRanking}{$\rho,\vpi,\vu, \hat{\vpi}, \mW$}
\Repeat 
\State Calculate $[\sigma_i(\vpi)]_{i\in[n]}$ by \eqref{eq: sigma and mu}
\State Calculate transition matrix $P(\vpi)$ by \eqref{eq: P}
\State $\vpi \gets$ steady-state distribution of $P(\vpi)$
\Until{Convergence}
\State \Return{$\vpi$}
\EndProcedure
\end{algorithmic}
\end{algorithm}

\noindent\textbf{Algorithm Overview and Complexity.} 
The algorithm is summarized in Algorithm~\ref{algo: ADMM}.
 We initialize $\vpi = \frac{1}{n} \vone \in \R^n$, $ \vu = \vzero \in \R^n$ and sample $\mtheta$ from a uniform distribution. Then, we iteratively: (1) optimize the scores $\vpi$ via Eq.~\eqref{lin pi} with Theorem~\ref{thm: ss} and power method; (2) optimize the parameters $\mtheta$ via Eq.~\eqref{lin theta} with GD; (3) update the dual parameter $\vu$ via Eq.~\eqref{dual params} until the scores converge. 

DeepSurv variants rely on the siamese neural networks to compute the negative log partial likelihood loss (see Eq.~\ref{eq: reweight deepsurv nll}). This involves a summation of $n$ terms, each further comprising $O(n)$ terms (as $|\mathcal{R}_i|$ is $O(n)$). Put differently, even with SGD, each batch of size $B$ loads features of $O(n)$ samples and copies the neural network $O(n)$ times (once for every term in $\mathcal{R}_i$). Overall, the time complexity of an epoch is $O(Pn)$ with the ascending order trick \citep{simon2011ascend}, where $P$ is the number of weights in the neural network, and the memory complexity is $O(PnB)$. On the other hand, in each epoch, the Alg.~\ref{algo: ADMM} (a) computes the intrinsic scores first via the power method, which is $O(n^2)$ and does not load model weights or sample features in memory, and (b) trains with a single neural network with complexity $O(Pn)$ with a standard cross-entropy loss. While the time complexity of the two methods in one epoch is comparable ($O(Pn)$ and $O(n^2)+ O(Pn)$), the spectral method reduces the memory complexity from $O(PnB)$ to $O(n^2)+O(PB)$. Thus, when $P = O(n)$, both methods have a time complexity of both methods $O(n^2)$, but \emph{the spectral method reduces the memory complexity by $B$}. When $P\gg n$, both methods again have the same time complexity $O(Pn)$ but \emph{the spectral method reduces the memory complexity by $n$}.



% \subsection{Extensions}
% \label{sec:extension}
% \subsection{Regressing CoxPH/DeepSurv}
% \label{subsec: regress DeepSurv}
% \noindent{\bf DeepSurv:} As a special case of weighted DeepSurv which has $\mW_{ij}=1, \forall i,j\in [n]$, it follows that there exists a closed-form solution for the augmented Lagrangian of \eqref{eq: DeepSurv Loss}
% \begin{align}
%     \min_{\vpi, \mtheta, \vu}\loss_{\rho}(\vpi, \mtheta, \vu
% )=& NLL(\dataset,\mtheta)+\vu (\vpi-h_{\mtheta}(\mX))\nonumber\\
% &+\rho\cdot \mathcal{D}_{KL}(\vpi||h_{\mtheta}(\mX)) \label{eq: Lagrangian deepsurv}
% \end{align}
% w.r.t $\vpi$ and it \emph{remains} the steady state distribution of a Markov Chain.

% % \begin{corollary}\label{cor:lag deepsurv}
% % The optimal solution to equation~\eqref{eq: Lagrangian deepsurv} is the steady state of the following MC
% % $\sum_{j\neq i}\vpi_j P_{ji}=\sum_{j\neq i} \vpi_i P_{ij}, \forall i\in [n]$, with transition rates as 
% % \begin{equation}\label{eq: P deepsurv}
% % P_{ji}=
% % \begin{cases}
% % \mu_{ji}+\frac{2\vpi_i \sigma_i(\vpi) \sigma_j(\vpi)}{\sum_{t\in [n]_-}\vpi_t \sigma_t(\vpi)-\sum_{t\in [n]_+}\vpi_t \sigma_t(\vpi)} & \textit{if } j \in [n]_+ \textit{ and } i\in [n]_-\\
% % \mu_{ji} & \textit{otherwise},\\
% % \end{cases}
% % \end{equation}
% % where 
% % \begin{align}
% % \sigma_i(\vpi)= &\rho \frac{\partial D_p(\vpi||h_{\mtheta}(\mx))}{\partial \vpi_i}+u^{(k)}_i\label{eq: sigma deepsurv}\\
% % \mu_{ji}=&\Delta_i \ind_{\{O_j> O_i\}} (\sum_{t\in R_i}  \vpi_t)^{-1} \label{eq: mu deepsurv}\\
% % W_i=\{\ell|i\in & R_\ell,c_\ell=i\},L_i=\{\ell|i\in R_{\ell},c_\ell\neq i\}
% % \end{align}
% % and we denote the partition of $[n]$ with $\sigma_i(\vpi)\geq 0$ and $\sigma_i(\vpi)\leq 0$ as $[n]_+$ and $[n]_-$.
% % \end{corollary}

% The other steps follow directly from Section~\ref{subsec: weighted deepsurv} as in Algorithm~\ref{algo: ADMM}.

% \noindent{\bf CoxPH:} Furthermore, CoxPH can be considered a single-layer network with an Identity activation function. Thus, it follows the argument of DeepSurv.


% The above reduction of \emph{weighted} CoxPH or DeepSurv model to a spectral solution enables us to extend this approach to a multitude of generalizations of CoxPH. We present these in more detail below. 

%\subsection{Regressing Deep Heterogenuous Hazard Model}







\begin{table}[!t]
\begin{center}
\begin{small}
\begin{tabular}{ccccccc}
\hline
Dataset& Feature & $n$ & $d$ &  $k$-fold  & Model structure &Censoring rate\\
\hline 
Synth Ads &\multirow{3}{*}{1D Low}   &{100,1K,10K} &50 & 5 & 2-6-layer MLP& 48.3\%\\
Support&        &9104 &34 & 5& 2-6-layer MLP& 68.1\%\\
METABRIC&   &1980 &8 & 5 & 2-6-layer MLP& 57.7\%\\
WHAS&          &1638 &5& 5 & 2-6-layer MLP& 42.1\%\\
\hline
DBCD &\multirow{3}{*}{1D High}         &295 &4919& 5 & 2-6-layer MLP& 73.2\%\\
DLBCL    &    &240 &7399& 5 & 2-6-layer MLP& 57.2\%\\
VDV     &      &78  &4705& 5  & 2-6-layer MLP& 43.5\%\\
\hline
 Lung1(3D) &3D         &422 &$68\! \times\! 512\! \times\! 512$&5 &  6-layer 3D-CNN& 11.4 \%\\
\hline
\end{tabular}
\end{small}
\end{center}
\caption{Overview of datasets and corresponding network structures explored.  1D High/Low denoting one-dimensional features of either high or low dimension, $n$ denotes the number of samples, $d$ denotes data dimension, 2-6-layer MLP hyperparameter explores MLPs from 2-layer to 6-layer. }
% Due to the limited data and high dimensionality of DLBCL, we implemented 10-fold for this specific dataset. 
\label{table: Datasets}
\end{table}


\begin{table*}[t]
\begin{center}
% \begin{small}
% \begin{sc}

\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccc}
\hline
Model&Algorithms &Features &  CI $\uparrow$& RMSE $\downarrow$  & iAUC $\uparrow$ & Memory& Time(s)\\
\hline 
% None & CoxPH\cite{aerts2014decoding} & Rad+Cli & 0.61* & $-$ & $-$ & &\\
2D-CNN & DeepSurv\cite{Haar2019}& Rad+Patches & 0.623*& $-$&0.64* &&\\
2D-CNN &  CE Loss\cite{Brag2023} &  Rad+Cli+Slices&  $-$ & $-$ &0.67* &&\\
3D-CNN &  Focal loss \cite{ZHENG2023109483} & Cli+ Cubes &$-$ & $-$ & 0.64*&&\\
2D-CNN & DeepSurv\cite{zhu2016deepconvsurv} & Patches &0.629*& $-$ & $-$&&\\
\hline
\multirow{8}{*}{3D-CNN}& \multirow{2}{*}{DeepSurv} & CT (FB)  & \ding{56}&\ding{56}   & \ding{56} & $>$80G&\\
& & CT (10\%B) &  0.580& 0.039& 0.622& 52GB&2038\\
&\multirow{2}{*}{DeepHit} & CT (FB)  & \ding{56} & \ding{56}  & \ding{56} & $>$80GB&\\
& & CT (10\%B) &  0.578& 0.252& 0.653& 65GB&?\\
&\multirow{2}{*}{MTLR} & CT (FB)  & \ding{56} & \ding{56} & \ding{56} & $>$80GB&\\
&  & CT (10\%B) & 0.539&0.104 & 0.55& 65GB& ?\\
&\multirow{2}{*}{CoxCC} & CT (FB) & \ding{56} & \ding{56}  & \ding{56} & $>$80GB&\\
& & CT (10\%B) & \ding{56}&  \ding{56} & \ding{56} & $>$80GB& \\
&\multirow{2}{*}{CoxTime} & CT (FB) & \ding{56} & \ding{56}   & \ding{56} & $>$80GB&\\
& & CT (10\%B) & \ding{56}  & \ding{56}  & \ding{56} & $>$80GB&\\
&Spectral &CT (FB) &\textbf{0.633}&\textbf{0.037}  &\textbf{0.697}& \textbf{31GB}& 2008\\
% &Spectral &Images(100\%batch) &  &  &  & &\\
% Plain Spectral \ding{70} & & & & & &  & &\\
% Classed Spectral & & & & & 0.61&  & &\\
\hline
\end{tabular}}
% \end{sc}
\caption{Overview of experiments on Lung1 dataset. We report previous SoTA results (top), operating on patches, cubes, or slices of the Lung1 CT scans, as well as on extracted 2D radiomic (Rad) features and clinical (Cli) features, and compare \textsc{Spectral} with five SOTA hazard models applied to the entire CT scan inputs (bottom), using mini-batch SGD. Additional batch sizes for DeepSurv and Spectral are reported in Fig.~\ref{fig: lung1}. * denotes the metrics as reported in original papers and $-$ denotes performance not reported. \ding{56} indicates that the method runs out of memory. FB denotes full batch.  \textsc{Spectral} operates on the whole input, surpassing SoTA with multi-modal inputs including extracted patches with manual annotation.  All competitor methods run out of memory beyond $10\%$ mini-batches on an 80GB A100 GPU, while \textsc{Spectral} works under the full-batch regime, improving performance.  } 
\label{table: Lung1 performance.}
% \end{small}
\end{center}
\end{table*}

%V100-SXM2-32GB

==> Preliminaries.tex <==
\section{Preliminaries}
\label{sec: preliminaries}

We provide a short review of survival analysis fundamentals; the subject is classic: we refer the interested reader to Aelen et al \cite{AalenBook} for a more thorough exposition on the subject, as well as to App.~\ref{app: related work}.

\subsection{Survival Analysis Problem Setup}
% while all $n$ feature vectors are denoted by a matrix $\mx \in \R^{n\times d}$
% We denote by $[n]=\{1,\dots,n\}$. 
Consider a dataset $\dataset$ comprising $n$ samples, each associated with a $d$-dimensional feature vector $\vx_i \in \R^d$. Each sample is additionally associated with an \emph{event time} $\et_i>0$ and a \emph{censoring time} $\ct_i>0$ (see Fig.~\ref{fig: illustration}). For example, each sample could correspond to a patient, the event time may denote a significant event in the patient's history (e.g., the patient is cured, exhibits a symptom, passes away, etc.), while the censoring time captures the length of the observation period: if the event happens \emph{after} the censoring time, we are not able to observe it.
% \begin{figure}[!t]
%   \centering
%   \includegraphics[width=\linewidth]{images/illustration.png}
%   \caption{}
%   \label{fig: illustration}
% \end{figure}




As shown in Fig~\ref{fig: illustration}, because we are not able to observe events outside the observation period, the dataset $\mathcal{D}$ is formally defined as $\mathcal{D}=\{\vx_i,\obt_i,\Delta_i\}^n_{i=1},\label{eq:dataset}$ where $O_i=\min(T_i,C_i)$ is the \emph{observation time} (either event or censoring) and $\Delta_i\equiv \ind_{\et_i\leq \ct_i}$ is the \emph{event indicator}, specifying whether the event was indeed observed. Note that $O_j=T_j$, i.e., an event time is observed, iff $\Delta_i=1$. The goal of survival analysis is to regress the distribution of the (only partially observed) times $\et_i$ from feature vectors $\vx_i$, using dataset $\mathcal{D}$. The act of censoring, i.e., the fact that events happening outside the observation period are not observed, distinguishes survival analysis from other forms of regression.



Typically, we express the distribution of event times via the so-called \emph{survival} and \emph{hazard} functions. The survival function is the complementary cdf, i.e.,
$S(t|\vx)=P(T>t|\vx)\label{eq:surv},$ i.e., it describes the likelihood that the event occurs after $t$. Given a sample $\vx$, the hazard function is:
\begin{align}\label{eq: hazard}
    \lambda(t|\vx)=\lim_{\delta \to 0} \frac{P(t\leq\! T\!\leq t\!+\!\delta|T\geq t,\vx)}{\delta}=\frac{f(t|\vx)}{S(t|\vx)}=-\frac{S'(t|\vx)}{S(t|\vx)},
\end{align}
where $f(t|\vx)=-S'(t|\vx)$ is the density function of $\et$ given $\vx$. Intuitively,
the hazard function captures the rate at which events occur, defined via the probability that an event happens in the infinitesimal interval $(t,t+\delta]$.  
Eq.~\eqref{eq: hazard} implies that we can express the survival function via the cumulative hazard via
%\begin{align}\label{eq: survival function}
 $   S(t|\vx)=\exp{\left(-\int_0^t \lambda(s|\vx)\, ds\right)}.$
%\end{align}
%Hence, we can obtain the hazard function from the survival function, and vice-versa.

\subsection{The CoxPH Model}
\label{subsec: hazard models}

One possible approach to learning feature-dependent hazard rates is to assume that event times follow a well-known distribution (e.g., exponential, Weibull, log-normal, etc.), and subsequently regress the parameters of this distribution from features using maximum likelihood estimation ~\citep{AalenBook}. However, as discussed in App.~\ref{app: related work}, the distribution selected by such a parametric approach may not fit the data well, introducing estimation bias. The Cox Proportional Hazard (CoxPH)~\citep{CoxPH1972} is a popular semi-parametric method that directly addresses this issue.
%
%{\bf Cox proportional hazard model (CoxPH) \citep{CoxPH1972}:}  Given the feature $\vx_i$, 
Formally, CoxPH assumes that the hazard rate has the form:
\begin{align}
    \lambda(t|\vx_i)=\lambda_0(t)e^{\mtheta^T \vx_i}, \quad i\in [n],\label{eq:coxhazard}
\end{align}
where $\lambda_0(\cdot)$ is a common baseline hazard function across all samples, and $\mtheta\in \mathbb{R}^d$ is a parameter vector. %Inference under CoxPH consists of two steps: (a) learning the parameter vector $\mtheta$ through MLE and (b) learning $\lambda_0(t)$ using a modified Nelson-Aalen estimate.
Parameter vector $\mtheta$ is learned by maximizing the so-called \emph{partial likelihood}:
\begin{align}
\mathcal{L}_{\mathtt{P}}(\dataset|\mtheta)&=\prod_{i=1}^n\left[\frac{\lambda(T_i|\vx_i)}{\sum_{j\in \mathcal{R}(T_i)}\lambda(T_i|\vx_j)}\right]^{\Delta_i}
% =&\prod_{i=1}^n\left[   \frac{ \lambda_0(t)e^{\mtheta^\top \vx_i}}{\sum_{j\in \mathcal{R}_i} \lambda_0(t) e^{\mtheta^\top \vx_j}}\right]^{\Delta_i}\\
\stackrel{\text{Eq.}~\eqref{eq:coxhazard}}{=}\prod_{i=1}^n\left[   \frac{ e^{\mtheta^\top \vx_i}}{\sum_{j\in \mathcal{R}(T_i)}  e^{\mtheta^\top \vx_j}}\right]^{\Delta_i}, \label{eq: CoxPH plik}
\end{align}
where $\mathcal{R}(t)\equiv \{j\in[n]: t<O_j\}$ be the set of at-risk samples at time $t$. Intuitively, this is called a partial likelihood because it characterizes the \emph{order} in which observed events occur, rather than the event times themselves. Indeed, the probability of the observed order of events is given by \eqref{eq: CoxPH plik}: this is because the probability that sample $i$ experiences the event before other at-risk samples at time $t$ are proportional to the hazard $\lambda(t|\vx_i)$. Crucially, as the hazard rate is given by Eq.~\eqref{eq:coxhazard}, the partial likelihood simplifies to Eq.~\eqref{eq: CoxPH plik}, that \emph{does not involve $\lambda_0$}. Hence, vector $\mtheta$ can be directly regressed from data \emph{separately} from $\lambda_0$, by minimizing the negative log-likelihood:
\begin{align}
\hat{\mtheta}=\argmin_{\mtheta}  \mathcal{L}_{\mathtt{NLL}}(\dataset,\mtheta) =\argmin_{\mtheta} \sum_{i=1}^n\Delta_i \left[\log \sum_{j\in \mathcal{R}(T_i)} e^{\mtheta^\top \vx_j}-\mtheta^\top \vx_i\right].\label{eq:nll}
\end{align}
This is typically obtained through standard techniques, e.g., gradient descent or Newton's method.
%
Having learned the parameter vector, the next step is to estimate the baseline hazard function. This can in general be done by an appropriately modified non-parametric method, such as Nelson-Aalen \cite{NelsonAalen1978} or Kaplan-Meier \cite{Kaplan1992}. For example, the lifelines package~\cite{davidson2019lifelines}  uses the Breslow estimator \cite{davidson2019lifelines, Xia2018Breslow}  to obtain the baseline hazard rate 
$\hat{\lambda}_0(t)= 1/\sum_{i\in \mathcal{R}(t)} h_{\mtheta}(\vx_i)$, with $h_{\mtheta}(\vx) = e^{\hat{\mtheta}^\top \vx_i}$. We review additional non-parametric methods in App.~\ref{app:non-parametric}.
% where $K(\cdot)$ is a kernel s.t.~$\int_{t\in\R} k(t)dt=1$,  $b$ is the so-called bandwidth of the smoothing, .
%Compared to Eq.~\eqref{eq: smoothing NA}, the cardinality of the at-risk set $Y(T_j)$ is replaced by the sum of the so-called relative hazard terms $e^{\hat{\mtheta}^\top \vx_i}$.
% This is known as the Breslow estimate of the cumulative hazard rate \cite{RamlauHansen1983SmoothingCP,AalenBook}; 
%we give a motivation and detailed explanation of constituent terms of \eqref{eq: smoothing Breslow} in Appendix~\ref{app:non-parametric}. 
%Note that, as a result, this estimate depends on the estimated parameters~$\hat{\mtheta}$.

The above end-to-end procedure has several benefits. Being semi-parametric allows regressing the hazard rate from features $\vx$ while maintaining the flexibility of fitting $\lambda_0$ to data through the Breslow estimate:  this significantly reduces bias compared to committing to, e.g., a log-normal distribution. Moreover, the parametrization via Eq.~\eqref{eq:coxhazard} naturally generalizes to several extensions, including deep models (see App.~\ref{app: extensions}). Most importantly, as discussed in the next section, a solution to  Eq.~\eqref{eq:nll} is obtainable via a spectral method~\cite{maystre2015fast,yildiz20a,yildiz21a}; establishing this is one of our main contributions.





==> Related.tex <==
\section{Related Work}
\label{sec: related work}
\paragraph{Survival Analysis.}
\begin{figure}[!t]
  \centering
  \subfloat[Survival analysis \label{fig: illustration}]{\input{plots/intro_plot}}
  \subfloat[Memory/Performance VS Batch size\label{fig: lung1}]{\input{plots/intro_plot3}}
  \subfloat[Time VS number of samples\label{fig: ads}]{\input{plots/experiment_ads}}
  \caption{a) An overview of the survival analysis process. Samples $\vx_i$, e.g., patients, are associated with the event times ($T_i$), e.g., a recovery, and the censor times ($C_i$): whichever occurs first is  observed ($O_i=\min(T_i, C_i)$). 
  %$\vx_1$ and $\vx_3$ are observed to experience the event at time $T_1$ and $T_3$ before their censorship. In contrast, $\vx_2$ is censored before the occurrence of events. 
  b)  Comparison between \textsc{Spectral} and DeepSurv on the Lung1 dataset under different batch sizes on an 80GB A100 GPU w.r.t. iAUC and memory consumption. The cross indicates DeepSurv runs out of memory, which happens beyond 10\%: memory consumption grows rapidly, while our method (\textsc{Spectral}) scales gracefully all the way to 100\% batch size, and attains better iAUC. c) The comparison between the proposed \textsc{Spectral} and \textsc{DeepSurv} on counting processes-based Synth Ads datasets against sample size ($n$). Spectral has significantly lower running time while attaining better iAUC: with 10K samples, Spectral takes less than 1\% of the time than DeepSurv. }\label{fig:teaser}
\end{figure}
Traditional statistical survival analysis methods are categorized as non-parametric, parametric, and semi-parametric~\cite{survivalcategory}. For completeness, we review all three in detail in App~\ref{app: related work}. In short, non-parametric methods, exemplified by the Kaplan-Meier \cite{Kaplan1992} and Nelson-Aalen estimators \cite{AalenBook}, estimate baseline hazard functions directly without making distributional assumptions. However, they do not explicitly capture the effects of features, limiting their ability to generalize out-of-sample. In contrast, parametric methods explicitly assume survival times follow parametrized distributions, such as exponentials \cite{WITTEN19927, jenkins2005survival}, Weibull, or log-normal~\cite{Wei1992TheAF}. In turn, distribution parameters can naturally be regressed from features \cite{AalenBook}. However, although parametric models offer simplicity and interpretability, they may have high bias and not fit the data well when the underlying distributional assumptions are violated.

Semi-parametric models, like  CoxPH~\cite{CoxPH1972}, incorporate features without assuming a specific form for the baseline hazard, striking a better bias-variance tradeoff.  Their popularity has led to numerous practical applications \cite{Katzman2018DeepSurvPT,mobadersany2018predicting, tran2021deep} as well as CoxPH deep variants from the machine learning community~\cite{zhu2016deepconvsurv, lee2018deephit, Deepsurvranking2019}. DeepSurv \cite{Katzman2018DeepSurvPT} replaces the linear predictor in CoxPH with a fully connected neural network \cite{SELU17} for predicting relative hazard risk. DeepConvSurv~\cite{zhu2016deepconvsurv} combines CoxPH with a CNN structure, to regress parameters from image datasets. CoxTime \cite{CoxTimeCC} stacks time into features to make the risk model time-dependent. DeepHit \citep{lee2018deephit} discretizes time into intervals and introduces a ranking loss to classify data into bins on the intervals.
%and it utilizes subnets to predict the event interval. 
Nnet-survival \citep{NNet} parameterizes discrete hazard rates by NNs and the hazard function is turned into the cumulative product of conditional probabilities based on intervals.
%  Besides, they propose CoxTime where time is stacked into features to make the risk model time-dependent.
% FastCPH \cite{yang2022fastcph} uses LassoNet \cite{lassonet21} within CoxPH to learn a sparse network to accelerate inference. 

Nevertheless,  the above methods either do not scale \cite{Katzman2018DeepSurvPT,zhu2016deepconvsurv,CoxTimeCC} or resort to mini-batch SGD ~\cite{NNet,lee2018deephit,CoxTimeCC}, which as discussed below reduces predictive performance. Scalability is hampered by training via gradient descent against the partial likelihood loss, yielding a Siamese network (SNN) penalty. As discussed in Sec.~\ref{sec: method}, this approach incurs significant computational and memory costs, as all samples, each associated with a copy of the model, can be loaded in a batch. As a result, both model and dataset sizes considered by prior art \cite{Katzman2018DeepSurvPT,zhu2016deepconvsurv,CoxTimeCC} are small: For example, DeepSurv only adopts a shallow two-layer Perceptron and the datasets contain hundreds of samples. 
%its variants can only handle patches of images rather than the whole image \cite{aerts2014decoding, Haar2019, Brag2023}. 
Approaches to resolve this include introducing mini-batch SGD (as done by Nnet-survival~\cite{NNet}, DeepHit~\cite{lee2018deephit}, and CoxCC~\cite{CoxTimeCC}) or decreasing input size by, e.g., handling patches of images rather than the whole image \cite{aerts2014decoding, Haar2019, Brag2023}: both come with a predictive performance degradation (see Fig.~\ref{fig: lung1} and Table.~\ref{table: Lung1 performance.}, respectively). Mini-batch SGD in particular suffers from introducing bias in gradient estimation (see App.\ref{app: biased est}, in contrast to SGD over traditional ML objectives that are separa.
%attempt to introduce mini-batch stochastic gradient descent to reduce the amount of SNN. However, the discrete essence of DeepHit inevitably loses information in discretization, and the Subnets that predict discrete event time are also of a Siamese structure. On the other hand, CoxCC and Nnet-survival still require the computation of a sufficiently large sampled risk set. Most importantly, although a mini-batch SGD can be implemented for the above methods with or without theoretical justification, the performance all degrades with the decrease of batch sizes {\color{red} as shown in Fig. X}. 
From another perspective, SODEN \cite{tang2022soden} expresses maximum likelihood estimation as a differential-equation-constrained optimization problem, which is tackled via numerical ODE solvers. However, even though SODEN allows mini-batch GD, Wu et al. later empirically observes that it incurs significantly worse computational/memory cost compared to the above-mentioned methods \cite{wu2023neural}.%The forward propagation requires solving an ODE numerically via a black-box ODE Solver while the backpropagation is based on numerically solving another augmented ODE. 

% Thus, modeling the whole distribution of event time introduces additional complexity. 

\paragraph{Rank Regression.}
In ranking regression problems \cite{guo19a, yildiz21a, yildizTKDD, RankSVM}, the goal is to regress a ranking among samples from sample features. RankSVM \cite{RankSVM} learns to rank via a linear Support Vector Machine, and it learns retrieval functions by analyzing the coefficients of each feature. RankRLS \cite{RankRLS} learns ranking with a regularized least-square ranking cost function based on a preference graph. Another line of work regresses from pairwise comparisons by executing maximum-likelihood estimation (MLE) based on the Bradley-Terry model \cite{bradley1952rank}, in either a shallow \cite{tian2019severity, guo2018experimental} or deep \cite{doughty2018s} setting. Several other papers \cite{han2018dateline, doughty2018s} regress from partial rankings via the Placket-Luce model \cite{PlackettLuce1975}, which generalizes Bradley-Terry. All the above methods apply the traditional Newton method to maximize the likelihood function, corresponding to training via siamese network penalty. This is both memory and computation-intensive. Yildiz et al \cite{yildiz20a, yildiz21a} accelerate computations and reduce the memory footprint by applying a spectral method proposed by Maystre and Grossglauser \cite{maystre2015fast} to the regression setting; we review both in App.~\ref{app: spectral}.

Leveraging the connection between the Placket-Luce model in ranking regression and the partial likelihood of the Cox model in survival analysis, we transfer the spectral method of Yildiz et al. to reduce memory costs and scale the Cox Proportional Hazard model. To account for (a) censoring and (b) the baseline hazard rate, we extend Yildiz et al. to a more general framework that works with both censorship and weights, enabling the extension to other survival analysis methods inlcuding CoxPH, its extensions, and several other survival analysis models such as the Accelerated Failure Model (AFT) scalable via the spectral method (see App.~\ref{app: extensions}). 

==> plots/experiment_ads.tex <==
\pgfplotsset{every axis/.append style={
    thick}}
\pgfplotsset{compat=1.13}





\begin{tikzpicture}
\begin{axis}[
        ylabel={Time (seconds)},
        y label style={color=darkgray,yshift=10pt},
        ylabel style={font=\tiny},
        ymin=1, ymax=40000,
        xmin=50, xmax=15000,
        xmode=log,
        ymode=log,
        log basis x={10},
        log basis y={10},
        axis y line*=right,
        axis x line=none,
        % ytick={1000, 2000},
        % yticklabels={1000, 2000, 3000},
        yticklabel style={text width=2em,align=left},
        % label style={font=\tiny},
        tick label style={font=\tiny}, 
        legend pos=north west,
        width=4.5cm,
        height=4.2cm
    ]
    % \addlegendimage{color=black, mark=halfdiamond*}
    % \addlegendentry{DeepSurv}
    % \addlegendimage{color=black, mark=triangle*}
    % \addlegendentry{Spectral}
    \addplot[
        color=darkgray,
        mark=halfdiamond*,
    ] table [x=n, y=Time, col sep=comma] {data1.csv};
    \addplot[
        color=darkgray,
        densely dashdotted,
        mark=halfcircle*,
        mark options={solid}
    ] table [x=n, y=Time, col sep=comma] {data2.csv};
    
    \end{axis}
    
    \begin{axis}[
        xlabel={Sample Size (n)},
        label style={font=\tiny},
        ylabel style={font=\tiny},
        ylabel={iAUC},
        y label style={color=brown,yshift=-15pt},
        ymin=0.5, ymax=0.8,
        xmin=50, xmax=15000,
        xmode=log,
        log basis x={10},
        legend pos=outer north east,
        axis y line*=left,
        yticklabel style={text width=2em,align=right},
        % label style={font=\tiny},
        tick label style={font=\tiny}, 
        % grid=major,
        width=4.5cm,
        height=4.2cm
    ]
    \addplot[
        color=brown,
        mark=halfdiamond*,
    ] table [x=n, y=AUC, col sep=comma] {data1.csv};
    \addplot[
        color=brown,
        densely dashdotted,,
        mark=halfcircle*,
        mark options={solid}
    ] table [x=n, y=AUC, col sep=comma] {data2.csv};
    % \addlegendentry{AUC}
    \end{axis}

    
\end{tikzpicture}



==> plots/intro_plot3.tex <==
\pgfplotsset{every axis/.append style={
    thick,
}}
    
\begin{tikzpicture}
    \begin{axis}[
        width=5cm,
        height=4.2cm,
        xlabel={$B$/$n$},
        xlabel style={font=\tiny},
        ylabel style={font=\tiny},
        xmin=0, xmax=1,
        ymin=0.32, ymax=0.75,
        % x dir=reverse,
        xtick={0,0.1, 0.2, 0.5,1},
        % ytick={0.3, 0.7},
        xticklabels = {$0$, $0.1$ ,$0.2$,  $0.5$, $1$},
        legend pos=north west,
        legend style={font=\fontsize{5}{5}\selectfont},
        % y axis line style=darkgray,
        % yticklabel style={darkgray},
        ylabel style={brown,yshift=-5pt},
        ylabel={iAUC},
        axis y line*=left,
        tick label style={font=\tiny},
        % extra y ticks={10,30,50,70},
        % extra y tick labels={10,30,50,70},
        % extra y tick style={grid=none,darkgray}
    ]
    \addplot[
        color=brown,
        % dashed,
        mark=halfdiamond*,
        mark options={solid}
    ]
    coordinates {
        (0.01, 0.52)(0.05,0.570) (0.1, 0.622) 
    };
    % \addlegendentry{DeepSurv}

    \addplot[
        color=brown,
        densely dashdotted,
        mark=halfcircle*,
        mark options={solid}
    ]
    coordinates {
        (0.01, 0.67)(0.05,0.69) (0.1, 0.69) (0.3, 0.69) (0.5, 0.699)  (1, 0.697)
    };
    
    % \addlegendentry{Spectral}
    
    \end{axis}

    \begin{axis}[
        width=5cm,
        height=4.2cm,
        % xlabel={$B$/$n$},
        xmin=0, xmax=1,
        ymin=25, ymax=80,
        % x dir=reverse,
        xtick={0,0.05, 0.1,0.3,0.5,1},
        ytick={20,40,60,80},
        xticklabels = {$0$, , , , $0.5$, $1$},
        legend pos=south east,
        legend style={font=\fontsize{5}{5}\selectfont, at={(0.73,0.66)},anchor=north},
        % legend style={}
        % y axis line style=brown,
        % yticklabel style={brown},
        tick label style={font=\tiny},
        ylabel style={font=\tiny},
        ylabel style={darkgray,yshift=5pt},
        ylabel={Memory (GB)},
        axis y line*=right,
    ]
    \addlegendimage{color=black, mark=halfdiamond*}
    \addlegendentry{DeepSurv}
    \addlegendimage{color=black, densely dashdotted, mark=halfcircle*,mark options={solid}}
    \addlegendentry{Spectral}
    
     

    \addplot[
        color=darkgray,
        mark=halfdiamond*,
        mark options={solid},
    ]
    coordinates {
        (0.01, 26)(0.05,31) (0.1, 56) 
    };

    \addplot[
        color=darkgray,
        dashed,
    ]
    coordinates {
         (0.1, 56) (0.2, 80) 
    };
    
    % \addlegendentry{DeepSurv}
      \addplot[
        color=black,
        mark=x,
        mark size = 5,
        mark options={line width=1pt},
    ]
    coordinates {
        (0.2,80)
    };
    
    \addplot[
        color=darkgray,
        densely dashdotted,
        mark=halfcircle*,
        mark options={solid},
    ]
    coordinates {
        (0.01, 30)(0.05,31) (0.1, 31) (0.3, 31) (0.5, 32) (1, 32)
    };
    
    \end{axis}
\end{tikzpicture}

